Nonequilibrium and Irreversibility

The work concentrates on relations, which are general and model independent in chaotic system, between time averages of a few (typically {\it very few}) observables. Equilibrium thermodynamics provides a guide and here is attempted to argue that the viewpoint of Sinai-Ruelle-Bowen can be regarded as a generalization to nonequilibrum phenomena of the theory of the ensembles proposing an answer to classical question like which distributions describe the statistics of stationary states (hence extend the analysis selecting canonical, or equivalent distributions, equilibrim between the uncountably many possibilities). The special name "Chaothic Hypothesis" (CH) is given to the above attempt and its mathematical meaning is discussed. General properties are presented and applied (eg. 'Fluctuation Theorem', 'Fluctuation Patterns', 'Pairing Symmetry') and related to the basic Time Reversal symmetry: which presents irreversibility as due to chaotic motion rather than to viscous forces. The case of a simple incompressible fluid is discussed in some detail. The possibility that CH is violated in various cases is considered: and in the end it is suggested that CH is the paradigm of chaotic evolution, as the harmonic oscillators are a paradigm of ordered motions, but of course {\it tertium datur}. The exposition is informal and often restricted to heuristic analysis, with detailed references to the literature and attention to numerical simulations and importance of stressing strongly the discrete models of Physics, trying to imitate the vision of Boltzmann, is widely considered.

==> a <==
\rm *.blg *.nav *.out *.snm *.toc *.aux *.tmp *.idx *.ilg *.ind *~ .*~ *.*~ *.dvi *.ps *.log 
latex N
bibtex N
latex N
latex N
bibtex N
makeindex N
latex N ;
latex N ; 
dvips N -oN.ps
ps2pdf N.ps
\rm *.blg *.nav *.out *.snm *.toc *.aux *.tmp *.idx *.ilg *.ind *~ .*~ *.*~ *.dvi *.ps *.log 

